VR-JEPA: Learning Contrastive-State Latent Guidance for Generation-based Video Reasoning

Reasoning through video generation offers a promising path toward visual intelligence by modeling latent visual states and their dynamics. However, current video generation models often lack explicit guidance on how these states should evolve, leaving generated trajectories prone to physical and structural inconsistencies that undermine reasoning reliability. While the Video Joint-Embedding Predictive Architecture (V-JEPA) provides rich spatiotemporal priors learned through latent prediction, these general priors do not naturally adapt to the logical reasoning capabilities required for complex visual tasks. To bridge this gap, we propose VR-JEPA, a framework that aligns the V-JEPA predictor with task-specific reasoning logic through localized contrastive-state learning and uses its predicted latent trajectories to guide video generation for visual reasoning. Specifically, (i) we pair successful trajectories with generated alternatives under the same input conditions and use discrepancies in their V-JEPA representations to identify informative states and tokens for localized contrastive supervision. (ii) We further equip the V-JEPA predictor with skill-specific experts trained on anchor-task data, allowing the model to adaptively specialize its shared spatiotemporal priors across diverse cognitive domains. Together with skill-specific experts, this contrastive supervision enables VR-JEPA to predict latent trajectories that provide task-specific logical guidance for video generation. Comprehensive experiments on the large-scale VBVR-Pro-Bench dataset demonstrate that VR-JEPA achieves an $11.33\%$ relative improvement over the cutting-edge generation-based reasoning baseline, significantly mitigating physical artifacts and enhancing logical consistency.

==> sections/05_limitations.tex <==
\section{Limitations}


==> tables/conditioning_schedule.tex <==
\begin{table}[h]
    \centering
    \small
    \setlength{\tabcolsep}{7pt}
    \renewcommand{\arraystretch}{1.05}

    \caption{
        \textbf{Ablation of the trajectory-conditioning schedule.}
        We compare injecting predicted latent trajectories during
high-noise denoising, low-noise denoising, or both, against
a baseline without trajectory conditioning.
ID and OOD task-success scores are reported on VBVR-Pro-Bench
as percentages; higher is better.
    }
    \label{tab:noise_ablation}

    \begin{tabular}{lcccc}
        \toprule
        \multirow{2}{*}{\textbf{Conditioning schedule}}
        & \multicolumn{2}{c}{\textbf{Conditioning stages}}
        & \multicolumn{2}{c}{\textbf{Task success (\%)}} \\
        \cmidrule(lr){2-3}
        \cmidrule(lr){4-5}

        & \textbf{High noise}
        & \textbf{Low noise}
        & \textbf{ID} $\uparrow$
        & \textbf{OOD} $\uparrow$ \\
        \midrule

        VBVR-Wan2.2
        & \xmarkg
        & \xmarkg
        & 55.4
        & 45.1 \\

        \addlinespace[2pt]

        High-noise only
        & \cmark
        & \xmarkg
        & 65.9
        & 46.1 \\

        Low-noise only
        & \xmarkg
        & \cmark
        & 56.2
        & 45.6 \\

        Dual-stage
        & \cmark
        & \cmark
        & \textbf{66.6}
        & \textbf{46.6} \\

        \bottomrule
    \end{tabular}
\end{table}
